Superconducting critical temperature and singlet and triplet pair functions of superconductor/normal-metal/ferromagnet trilayers

We calculate the superconducting critical temperature $T_c$, the singlet pair function $\Psi^+(x)$, and triplet pair function $\Psi^-(x)$ of superconductor/normal metal/ferromagnet (S/N/F) trilayers using the linearized Usadel equation near $T_c$. The Green's function method developed by Fominov $et al.$ for the S/F bilayers is extended to the S/N/F trilayer systems. The S of the trilayers is taken to be an s-wave singlet pairing superconductor, and the S/N and N/F interfaces are modeled in terms of the interface resistances parameterized, respectively, by $\gamma_b^{SN}$ and $\gamma_b^{NF}$. We present the $T_c$, $\Psi^+(x)$, and $\Psi^-(x)$ for typical $\gamma_b^{SN}$, $\gamma_b^{NF}$, and the exchange energy $ E_{ex}$: (a) For a small (large) $\gamma_b^{NF}$, $T_c$ of S/N/F trilayers, as $d_N$ is increased, increases (decreases) on the length scale of N coherence length $\xi_N$ with a discontinuity at $d_N=0$ due to a boundary condition mismatch. (b) $T_c(d_F)$ shows a non-monotonic behavior like S/F bilayers with a weakened shallow dip. (c) The odd frequency triplet component $\Psi^-(x)$, induced by $E_{ex}$ and proximity effects, has a maximum near the N/F interface and decreases on the length scale $\xi_{ex}$ in F. It also penetrates into N and S regions on the length scale $\xi_N$ and $\xi_S$, respectively. Based on these results we make comments on the experimental observation of the odd triplet components and the recent $T_c$ measurements in Nb/Au/CoFe trilayer systems.

==> newdefinition.tex <==
\def \ba {\begin{eqnarray}}
\def \ea {\end{eqnarray}}
\def \bc {\begin{cases}}
\def \ec {\end{cases}}
\def \be {\begin{equation}}
\def \ee {\end{equation}}
\def \barr {\begin{array}}
\def \earr {\end{array}}
\def \bi {\begin{itemize}}
\def \ei {\end{itemize}}
\def \bmat {\left(\begin{array}}
\def \emat {\end{array}\right)}
\def \tight {\!\!\!}
\def \vr {\vec r}
\def \vcr {\vec R}
\def \vx {\vec x}
\def \vi {\vec i}
\def \vp {\vec p}
\def \vcp {\vec P}
\def \vk {\vec k}
\def \vv {\vec v}
\def \vq {\vec q}
\def \wt {\widetilde}
\def \wh {\widehat}
\def \ra {\rightarrow}
\def \ua {\uparrow}
\def \da {\downarrow}
\def \sch {\rm Schr{\ddot o}dinger}

